Discrete Energy Minimization, beyond Submodularity: Applications and Approximations

In this thesis I explore challenging discrete energy minimization problems that arise mainly in the context of computer vision tasks. This work motivates the use of such "hard-to-optimize" non-submodular functionals, and proposes methods and algorithms to cope with the NP-hardness of their optimization. Consequently, this thesis revolves around two axes: applications and approximations. The applications axis motivates the use of such "hard-to-optimize" energies by introducing new tasks. As the energies become less constrained and structured one gains more expressive power for the objective function achieving more accurate models. Results show how challenging, hard-to-optimize, energies are more adequate for certain computer vision applications. To overcome the resulting challenging optimization tasks the second axis of this thesis proposes approximation algorithms to cope with the NP-hardness of the optimization. Experiments show that these new methods yield good results for representative challenging problems.

==> acknowledge.tex <==

\chapter*{Acknowledgments}

To Daffy

To Alma, Mica and Ruth

To my Parents

To Michal and Meirav


Eli Schechtmann and Aseem Agrawala - Adobe 

Carsten Rother, Sebastian Nowozin, Toby Sharp and Pushmeet Kohli - MSRC


\clearpage 
